Latent Class Concept Bottleneck Models

Concept bottleneck models (CBMs) are interpretable image models that predict a target through a layer of human-understandable concepts. Because the prediction depends on the input only through these concepts, a user can correct mispredicted concepts at test time and thereby change the prediction. Standard CBMs, however, treat concepts as independent, so a correction never propagates to other concepts. Recently, Stochastic CBMs (SCBMs) have modeled concept dependencies with a Gaussian on the concept logits, but their interventions rely on a heuristic rather than exact conditioning. We propose Latent Class CBMs (LC-CBMs), which model the concepts as an input-dependent mixture of product-Bernoulli distributions. This gives an exact likelihood and exact Bayesian interventions. Across synthetic data, CUB, CIFAR-10 and CIFAR-100, LC-CBM matches or outperforms the baselines in target and concept accuracy, and achieves the most effective interventions on all four datasets. We further show that the latent-class structure is not specific to CBMs: added to concept embedding models, it also improves their interventions.

==> tables/ablation.tex <==
\begin{tabular}{llcccc}
\toprule
Dataset & Auxiliary head loss & Concept acc. & Target acc. & Concept ECE$\downarrow$ & AUC (unc.) \\
\midrule
\multirow{2}{*}{CUB} & With & \textbf{96.07{\scriptsize$\pm$0.05}} & \textbf{72.35{\scriptsize$\pm$0.40}} & \textbf{1.09{\scriptsize$\pm$0.04}} & \textbf{99.31{\scriptsize$\pm$0.01}} \\
 & Without & 96.00{\scriptsize$\pm$0.05} & 71.63{\scriptsize$\pm$0.54} & 1.11{\scriptsize$\pm$0.04} & 97.99{\scriptsize$\pm$0.29} \\
\midrule
\multirow{2}{*}{CIFAR-10} & With & 86.47{\scriptsize$\pm$0.02} & \textbf{71.47{\scriptsize$\pm$0.29}} & \textbf{0.97{\scriptsize$\pm$0.07}} & \textbf{84.45{\scriptsize$\pm$0.06}} \\
 & Without & \textbf{86.48{\scriptsize$\pm$0.03}} & 71.42{\scriptsize$\pm$0.11} & 0.99{\scriptsize$\pm$0.07} & 82.68{\scriptsize$\pm$0.07} \\
\midrule
\multirow{2}{*}{CIFAR-100} & With & \textbf{84.59{\scriptsize$\pm$0.05}} & \textbf{39.90{\scriptsize$\pm$0.85}} & \textbf{3.39{\scriptsize$\pm$0.07}} & \textbf{51.03{\scriptsize$\pm$0.27}} \\
 & Without & 84.46{\scriptsize$\pm$0.01} & 39.48{\scriptsize$\pm$0.37} & 3.52{\scriptsize$\pm$0.08} & 42.52{\scriptsize$\pm$0.33} \\
\bottomrule
\end{tabular}

==> tables/efficiency.tex <==
\begin{tabular}{llrrrr}
\toprule
$C$ & Concept layer & Parameters & Train step (ms) & Train memory (MB) & Intervention step (ms) \\
\midrule
100 & CBM & 25,700 & 3.8 & 42 & 0.1 \\
100 & SCBM (amortized) & 1,323,550 & 5.9 & 73 & 764.6 \\
100 & LC-CBM (K=200) & 97,100 & 10.3 & 558 & 1.3 \\
300 & CBM & 77,100 & 5.0 & 133 & 0.1 \\
300 & SCBM (amortized) & 11,680,650 & 11.1 & 385 & 790.0 \\
300 & LC-CBM (K=200) & 188,500 & 29.1 & 1869 & 4.5 \\
900 & CBM & 231,300 & 7.1 & 596 & 0.1 \\
900 & SCBM (amortized) & 104,431,950 & 110.8 & 2944 & 1154.3 \\
900 & LC-CBM (K=200) & 462,700 & \multicolumn{3}{c}{exceeds per-job memory cap of the benchmark} \\
\bottomrule
\end{tabular}


==> tables/eig.tex <==
\begin{tabular}{llcccc}
\toprule
Dataset & Model & AUC (unc.) & AUC (EIG) & Acc@5 (unc.) & Acc@5 (EIG) \\
\midrule
\multirow{3}{*}{Synthetic} & Hard CBM & 69.12{\scriptsize$\pm$3.12} & 74.09{\scriptsize$\pm$3.47} & 58.3 & 62.6 \\
 & Amortized SCBM$^\ddagger$ & 73.26{\scriptsize$\pm$3.73} & 75.29{\scriptsize$\pm$3.75} & 62.0 & 68.6 \\
 & \textbf{LC-CBM} & \textbf{75.50{\scriptsize$\pm$3.34}} & \textbf{78.27{\scriptsize$\pm$3.69}} & \textbf{62.9} & \textbf{71.6} \\
\midrule
\multirow{3}{*}{CUB} & Hard CBM & 96.03{\scriptsize$\pm$0.12} & 96.24{\scriptsize$\pm$0.08} & 77.1 & 77.2 \\
 & Amortized SCBM$^\ddagger$ & 98.04{\scriptsize$\pm$0.06} & 97.72{\scriptsize$\pm$0.08} & 87.9 & 84.4 \\
 & \textbf{LC-CBM} & \textbf{99.32{\scriptsize$\pm$0.01}} & \textbf{99.27{\scriptsize$\pm$0.03}} & \textbf{97.0} & \textbf{97.0} \\
\midrule
\multirow{3}{*}{CIFAR-10} & Hard CBM & 81.85{\scriptsize$\pm$0.09} & 83.27{\scriptsize$\pm$0.06} & 71.0 & 76.0 \\
 & Amortized SCBM$^\ddagger$ & 82.98{\scriptsize$\pm$0.03} & 84.23{\scriptsize$\pm$0.06} & 71.4 & 78.7 \\
 & \textbf{LC-CBM} & \textbf{84.48{\scriptsize$\pm$0.04}} & \textbf{85.42{\scriptsize$\pm$0.03}} & \textbf{74.9} & \textbf{81.0} \\
\bottomrule
\end{tabular}

==> tables/frozen.tex <==
\begin{tabular}{llccccc}
\toprule
Dataset ($C$) & Concept layer & Concept acc. & Target acc. & Concept ECE & AUC (unc.) & Seeds \\
\midrule
\multirow{4}{*}{CIFAR-10 (143)} & Hard CBM$^\dagger$ & 87.70{\scriptsize$\pm$0.04} & 88.74{\scriptsize$\pm$0.17} & 3.54{\scriptsize$\pm$0.06} & 86.22{\scriptsize$\pm$0.02} & 5 \\
 & Global SCBM$^\dagger$ & 87.86{\scriptsize$\pm$0.02} & 89.32{\scriptsize$\pm$0.17} & 1.93{\scriptsize$\pm$0.07} & 86.35{\scriptsize$\pm$0.04} & 5 \\
 & Amortized SCBM$^\dagger$ & 87.82{\scriptsize$\pm$0.01} & 89.45{\scriptsize$\pm$0.20} & 2.08{\scriptsize$\pm$0.05} & 86.23{\scriptsize$\pm$0.07} & 5 \\
 & \textbf{LC-CBM (ours)} & \textbf{88.32{\scriptsize$\pm$0.01}} & \textbf{90.11{\scriptsize$\pm$0.24}} & \textbf{0.87{\scriptsize$\pm$0.03}} & \textbf{86.57{\scriptsize$\pm$0.08}} & 5 \\
\midrule
\multirow{4}{*}{CUB (112)} & Hard CBM$^\dagger$ & 91.15{\scriptsize$\pm$0.01} & 50.32{\scriptsize$\pm$0.46} & 1.89{\scriptsize$\pm$0.03} & 86.24{\scriptsize$\pm$0.49} & 5 \\
 & Global SCBM$^\dagger$ & 91.01{\scriptsize$\pm$0.02} & 50.37{\scriptsize$\pm$0.51} & 1.17{\scriptsize$\pm$0.04} & 84.11{\scriptsize$\pm$0.63} & 5 \\
 & Amortized SCBM$^\dagger$ & 88.40{\scriptsize$\pm$0.83} & 30.13{\scriptsize$\pm$10.19} & 2.68{\scriptsize$\pm$0.37} & 46.33{\scriptsize$\pm$17.62} & 5 \\
 & \textbf{LC-CBM (ours)} & \textbf{94.86{\scriptsize$\pm$0.02}} & \textbf{64.28{\scriptsize$\pm$0.34}} & \textbf{0.81{\scriptsize$\pm$0.01}} & \textbf{99.16{\scriptsize$\pm$0.00}} & 5 \\
\midrule
\multirow{4}{*}{CUB-CLIP (370)} & Hard CBM$^\dagger$ & 87.23{\scriptsize$\pm$0.04} & 42.20{\scriptsize$\pm$0.37} & 3.08{\scriptsize$\pm$0.05} & 43.45{\scriptsize$\pm$0.17} & 5 \\
 & Global SCBM$^\dagger$ & \textbf{87.76{\scriptsize$\pm$0.01}} & 46.30{\scriptsize$\pm$0.37} & \textbf{1.56{\scriptsize$\pm$0.01}} & 39.97{\scriptsize$\pm$0.10} & 5 \\
 & Amortized SCBM$^\dagger$ & 85.17{\scriptsize$\pm$0.62} & 20.26{\scriptsize$\pm$3.77} & 3.81{\scriptsize$\pm$1.15} & 16.54{\scriptsize$\pm$2.70} & 4 \\
 & \textbf{LC-CBM (ours)} & 87.65{\scriptsize$\pm$0.03} & \textbf{47.75{\scriptsize$\pm$0.29}} & 1.67{\scriptsize$\pm$0.03} & \textbf{45.76{\scriptsize$\pm$0.12}} & 5 \\
\midrule
\multirow{4}{*}{CIFAR-100 (892)} & Hard CBM$^\dagger$ & 86.76{\scriptsize$\pm$0.02} & 68.63{\scriptsize$\pm$0.48} & 2.89{\scriptsize$\pm$0.02} & 70.85{\scriptsize$\pm$0.28} & 3 \\
 & Global SCBM$^\dagger$ & 86.91{\scriptsize$\pm$0.02} & 69.28{\scriptsize$\pm$0.10} & 1.59{\scriptsize$\pm$0.19} & 71.44{\scriptsize$\pm$0.25} & 3 \\
 & Amortized SCBM$^\dagger$ & 86.61{\scriptsize$\pm$0.07} & 64.97{\scriptsize$\pm$0.09} & 1.62{\scriptsize$\pm$0.26} & 68.00{\scriptsize$\pm$0.17} & 3 \\
 & \textbf{LC-CBM (ours)} & \textbf{86.97{\scriptsize$\pm$0.00}} & \textbf{69.36{\scriptsize$\pm$0.28}} & \textbf{1.41{\scriptsize$\pm$0.02}} & \textbf{71.65{\scriptsize$\pm$0.07}} & 3 \\
\bottomrule
\end{tabular}


==> tables/interp.tex <==
\begin{tabular}{lcccccc}
\toprule
Model & $K$ & Classes used & Mean $\max_k\pi_k$ & Purity & NMI & Latent classes per label \\
\midrule
CIFAR-10 (frozen R50) & 200 & 198 & 0.22 & 0.87 & 0.53 & 60.1 (max 82) \\
CIFAR-10 (end-to-end) & 200 & 191 & 0.16 & 0.70 & 0.38 & 96.6 (max 119) \\
CUB (end-to-end) & 200 & 198 & 0.79 & 0.72 & 0.82 & 5.9 (max 15) \\
CUB-CLIP (frozen R50) & 50 & 50 & 0.30 & 0.14 & 0.50 & 6.7 (max 15) \\
CUB (frozen R50) & 200 & 198 & 0.69 & 0.64 & 0.77 & 7.3 (max 18) \\
\bottomrule
\end{tabular}


==> tables/k1.tex <==
\begin{tabular}{llccccc}
\toprule
Dataset & Model & Concept acc. & Target acc. & Joint NLL & AUC (unc.) & $n{=}5$ (unc.) \\
\midrule
\multirow{4}{*}{CUB} & Hard CBM (SCBM defaults) & 95.18{\scriptsize$\pm$0.16} & 67.64{\scriptsize$\pm$0.85} & 16.56 & 96.03{\scriptsize$\pm$0.12} & 77.1 \\
 & Hard CBM + LC training recipe & 94.97{\scriptsize$\pm$0.06} & 67.70{\scriptsize$\pm$0.16} & 15.24 & 96.85{\scriptsize$\pm$0.25} & 81.2 \\
 & LC-CBM, $K=1$ & 94.58{\scriptsize$\pm$0.05} & 66.38{\scriptsize$\pm$0.08} & 15.87 & 96.90{\scriptsize$\pm$0.03} & 80.4 \\
 & \textbf{LC-CBM}, selected $K$ & 96.12{\scriptsize$\pm$0.06} & 72.76{\scriptsize$\pm$0.21} & 1.21 & 99.32{\scriptsize$\pm$0.01} & 97.0 \\
\midrule
\multirow{4}{*}{CIFAR-10} & Hard CBM (SCBM defaults) & 85.43{\scriptsize$\pm$0.08} & 69.12{\scriptsize$\pm$0.28} & 49.13 & 81.85{\scriptsize$\pm$0.09} & 71.0 \\
 & Hard CBM + LC training recipe & 86.33{\scriptsize$\pm$0.02} & 70.35{\scriptsize$\pm$0.51} & 43.67 & 83.26{\scriptsize$\pm$0.07} & 72.4 \\
 & LC-CBM, $K=1$ & 86.18{\scriptsize$\pm$0.00} & 69.22{\scriptsize$\pm$0.42} & 44.02 & 83.07{\scriptsize$\pm$0.08} & 71.7 \\
 & \textbf{LC-CBM}, selected $K$ & 86.49{\scriptsize$\pm$0.02} & 71.41{\scriptsize$\pm$0.10} & 33.20 & 84.48{\scriptsize$\pm$0.04} & 74.9 \\
\midrule
\multirow{4}{*}{CUB (frozen R50)} & Hard CBM (SCBM defaults) & 91.15{\scriptsize$\pm$0.00} & 50.41{\scriptsize$\pm$0.44} & 24.24 & 86.18{\scriptsize$\pm$0.39} & 62.6 \\
 & Hard CBM + LC training recipe & 91.14{\scriptsize$\pm$0.01} & 52.84{\scriptsize$\pm$0.06} & 24.25 & 95.32{\scriptsize$\pm$0.27} & 71.7 \\
 & LC-CBM, $K=1$ & 90.91{\scriptsize$\pm$0.02} & 49.78{\scriptsize$\pm$0.13} & 24.73 & 94.83{\scriptsize$\pm$0.03} & 69.5 \\
 & \textbf{LC-CBM}, selected $K$ & 94.87{\scriptsize$\pm$0.02} & 64.09{\scriptsize$\pm$0.25} & 1.41 & 99.16{\scriptsize$\pm$0.01} & 96.7 \\
\bottomrule
\end{tabular}


==> tables/ksens.tex <==
\begin{tabular}{lcccccc}
\toprule
Dataset & $K$ & Concept acc. & Target acc. & Joint NLL & AUC (unc.) & Seeds \\
\midrule
\multirow{6}{*}{CUB (frozen R50)} & 10 & 91.39{\scriptsize$\pm$0.06} & 52.21{\scriptsize$\pm$0.40} & 18.69 & 96.51{\scriptsize$\pm$0.14} & 3 \\
 & 20 & 91.68{\scriptsize$\pm$0.03} & 51.99{\scriptsize$\pm$0.37} & 16.16 & 96.75{\scriptsize$\pm$0.33} & 3 \\
 & 50 & 92.53{\scriptsize$\pm$0.06} & 54.72{\scriptsize$\pm$0.47} & 10.92 & 97.37{\scriptsize$\pm$0.33} & 3 \\
 & 100 & 93.63{\scriptsize$\pm$0.03} & 58.15{\scriptsize$\pm$0.23} & 5.78 & 98.39{\scriptsize$\pm$0.02} & 3 \\
 & 200 & 94.87{\scriptsize$\pm$0.01} & 64.18{\scriptsize$\pm$0.36} & 1.41 & 99.15{\scriptsize$\pm$0.00} & 3 \\
 & 500 & 94.84{\scriptsize$\pm$0.03} & 63.91{\scriptsize$\pm$0.49} & 1.67 & 98.91{\scriptsize$\pm$0.29} & 3 \\
\midrule
\multirow{6}{*}{CIFAR-10 (frozen R50)} & 10 & 88.17{\scriptsize$\pm$0.01} & 89.64{\scriptsize$\pm$0.05} & 31.61 & 87.00{\scriptsize$\pm$0.03} & 3 \\
 & 20 & 88.18{\scriptsize$\pm$0.01} & 89.65{\scriptsize$\pm$0.12} & 31.25 & 86.90{\scriptsize$\pm$0.05} & 3 \\
 & 50 & 88.24{\scriptsize$\pm$0.01} & 89.97{\scriptsize$\pm$0.05} & 30.82 & 86.54{\scriptsize$\pm$0.06} & 3 \\
 & 100 & 88.28{\scriptsize$\pm$0.02} & 89.96{\scriptsize$\pm$0.03} & 30.44 & 86.52{\scriptsize$\pm$0.03} & 3 \\
 & 200 & 88.32{\scriptsize$\pm$0.02} & 90.10{\scriptsize$\pm$0.11} & 30.24 & 86.59{\scriptsize$\pm$0.10} & 3 \\
 & 500 & 88.35{\scriptsize$\pm$0.01} & 90.29{\scriptsize$\pm$0.28} & 30.48 & 86.67{\scriptsize$\pm$0.07} & 3 \\
\bottomrule
\end{tabular}


==> tables/lf/alpha_c100.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{CIFAR-100, sparse labels: effect of the concept-loss weight $\alpha$. For every model and setting the validation task NLL selects the smallest candidate $\alpha=0.03$ (candidates $\{1,0.3,0.1,0.03\}$). Lower $\alpha$ raises task accuracy but lowers concept fidelity (C-AUROC$_B$: mean per-concept AUROC of the predicted concept probabilities).}
\label{tab:lf_alpha}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccccc}
\toprule
Labels & Model & Acc@0 & Acc@50 & Int-AUC & C-AUROC$_B$ & Imp-AUROC & Joint NLL$\downarrow$ \\
\midrule
\multirow{7}{*}{$\rho=0.1$} & LC-CBM (ours) ($\alpha{=}1$) & 0.609{\scriptsize$\pm$0.007} & 0.626{\scriptsize$\pm$0.009} & 0.634{\scriptsize$\pm$0.009} & \textbf{0.856{\scriptsize$\pm$0.000}} & \textbf{0.947{\scriptsize$\pm$0.003}} & \textbf{230.0{\scriptsize$\pm$0.1}} \\
 & LC-CBM (ours) ($\alpha{=}0.03$) & \textbf{0.696{\scriptsize$\pm$0.004}} & \textbf{0.708{\scriptsize$\pm$0.005}} & \textbf{0.712{\scriptsize$\pm$0.004}} & 0.807{\scriptsize$\pm$0.003} & 0.930{\scriptsize$\pm$0.004} & 266.2{\scriptsize$\pm$0.5} \\
 & LF-SCBM (IS) ($\alpha{=}1$) & 0.589{\scriptsize$\pm$0.002} & 0.602{\scriptsize$\pm$0.001} & 0.611{\scriptsize$\pm$0.002} & 0.851{\scriptsize$\pm$0.001} & 0.943{\scriptsize$\pm$0.004} & 239.8{\scriptsize$\pm$0.2} \\
 & LF-SCBM (IS) ($\alpha{=}0.03$) & 0.689{\scriptsize$\pm$0.000} & 0.697{\scriptsize$\pm$0.002} & 0.700{\scriptsize$\pm$0.002} & 0.804{\scriptsize$\pm$0.001} & 0.924{\scriptsize$\pm$0.001} & 314.5{\scriptsize$\pm$0.7} \\
 & CBM ($\alpha{=}1$) & 0.603{\scriptsize$\pm$0.004} & 0.616{\scriptsize$\pm$0.005} & 0.625{\scriptsize$\pm$0.005} & 0.850{\scriptsize$\pm$0.000} & 0.937{\scriptsize$\pm$0.000} & 277.7{\scriptsize$\pm$0.3} \\
 & CBM ($\alpha{=}0.03$) & 0.695{\scriptsize$\pm$0.003} & 0.701{\scriptsize$\pm$0.002} & 0.705{\scriptsize$\pm$0.003} & 0.813{\scriptsize$\pm$0.001} & 0.922{\scriptsize$\pm$0.001} & 316.7{\scriptsize$\pm$0.2} \\
 & LF-CBM & 0.634{\scriptsize$\pm$0.002} & 0.608{\scriptsize$\pm$0.000} & 0.582{\scriptsize$\pm$0.003} & 0.581{\scriptsize$\pm$0.001} & 0.885{\scriptsize$\pm$0.000} & -- \\
\midrule
\multirow{7}{*}{$\rho=0.03$} & LC-CBM (ours) ($\alpha{=}1$) & 0.592{\scriptsize$\pm$0.004} & 0.601{\scriptsize$\pm$0.005} & 0.603{\scriptsize$\pm$0.005} & \textbf{0.827{\scriptsize$\pm$0.001}} & \textbf{0.938{\scriptsize$\pm$0.002}} & \textbf{264.2{\scriptsize$\pm$0.2}} \\
 & LC-CBM (ours) ($\alpha{=}0.03$) & \textbf{0.695{\scriptsize$\pm$0.003}} & \textbf{0.700{\scriptsize$\pm$0.004}} & \textbf{0.699{\scriptsize$\pm$0.003}} & 0.729{\scriptsize$\pm$0.004} & 0.888{\scriptsize$\pm$0.002} & 396.7{\scriptsize$\pm$0.2} \\
 & LF-SCBM (IS) ($\alpha{=}1$) & 0.579{\scriptsize$\pm$0.006} & 0.586{\scriptsize$\pm$0.006} & 0.589{\scriptsize$\pm$0.005} & 0.821{\scriptsize$\pm$0.001} & 0.931{\scriptsize$\pm$0.002} & 281.1{\scriptsize$\pm$0.6} \\
 & LF-SCBM (IS) ($\alpha{=}0.03$) & 0.691{\scriptsize$\pm$0.004} & 0.691{\scriptsize$\pm$0.004} & 0.690{\scriptsize$\pm$0.003} & 0.698{\scriptsize$\pm$0.002} & 0.859{\scriptsize$\pm$0.001} & 491.9{\scriptsize$\pm$1.3} \\
 & CBM ($\alpha{=}1$) & 0.576{\scriptsize$\pm$0.011} & 0.581{\scriptsize$\pm$0.011} & 0.588{\scriptsize$\pm$0.010} & 0.820{\scriptsize$\pm$0.000} & 0.927{\scriptsize$\pm$0.000} & 301.6{\scriptsize$\pm$1.2} \\
 & CBM ($\alpha{=}0.03$) & \textbf{0.695{\scriptsize$\pm$0.002}} & 0.695{\scriptsize$\pm$0.000} & 0.696{\scriptsize$\pm$0.002} & 0.716{\scriptsize$\pm$0.003} & 0.875{\scriptsize$\pm$0.001} & 445.8{\scriptsize$\pm$1.7} \\
 & LF-CBM & 0.623{\scriptsize$\pm$0.002} & 0.595{\scriptsize$\pm$0.002} & 0.569{\scriptsize$\pm$0.002} & 0.552{\scriptsize$\pm$0.001} & 0.882{\scriptsize$\pm$0.000} & -- \\
\midrule
\multirow{7}{*}{10\% images} & LC-CBM (ours) ($\alpha{=}1$) & 0.612{\scriptsize$\pm$0.012} & 0.619{\scriptsize$\pm$0.017} & 0.622{\scriptsize$\pm$0.017} & 0.830{\scriptsize$\pm$0.004} & 0.933{\scriptsize$\pm$0.001} & \textbf{236.3{\scriptsize$\pm$2.9}} \\
 & LC-CBM (ours) ($\alpha{=}0.03$) & \textbf{0.695{\scriptsize$\pm$0.006}} & \textbf{0.699{\scriptsize$\pm$0.006}} & \textbf{0.697{\scriptsize$\pm$0.006}} & 0.772{\scriptsize$\pm$0.008} & 0.821{\scriptsize$\pm$0.012} & 260.0{\scriptsize$\pm$2.5} \\
 & LF-SCBM (IS) ($\alpha{=}1$) & 0.566{\scriptsize$\pm$0.011} & 0.579{\scriptsize$\pm$0.010} & 0.585{\scriptsize$\pm$0.010} & \textbf{0.840{\scriptsize$\pm$0.000}} & \textbf{0.942{\scriptsize$\pm$0.003}} & 243.2{\scriptsize$\pm$0.5} \\
 & LF-SCBM (IS) ($\alpha{=}0.03$) & 0.683{\scriptsize$\pm$0.008} & 0.686{\scriptsize$\pm$0.010} & 0.686{\scriptsize$\pm$0.011} & 0.793{\scriptsize$\pm$0.001} & 0.920{\scriptsize$\pm$0.005} & 287.8{\scriptsize$\pm$1.2} \\
 & CBM ($\alpha{=}1$) & 0.537{\scriptsize$\pm$0.012} & 0.549{\scriptsize$\pm$0.013} & 0.562{\scriptsize$\pm$0.012} & 0.837{\scriptsize$\pm$0.001} & 0.932{\scriptsize$\pm$0.000} & 288.4{\scriptsize$\pm$0.3} \\
 & CBM ($\alpha{=}0.03$) & 0.684{\scriptsize$\pm$0.005} & 0.687{\scriptsize$\pm$0.004} & 0.691{\scriptsize$\pm$0.005} & 0.811{\scriptsize$\pm$0.001} & 0.920{\scriptsize$\pm$0.000} & 324.5{\scriptsize$\pm$0.1} \\
 & LF-CBM & 0.627{\scriptsize$\pm$0.002} & 0.598{\scriptsize$\pm$0.004} & 0.573{\scriptsize$\pm$0.003} & 0.585{\scriptsize$\pm$0.002} & 0.885{\scriptsize$\pm$0.000} & -- \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/lf/fidelity_c10.tex <==
\begin{table*}[h]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{CIFAR-10: concept fidelity against the training annotator (C-AUROC$_B$, CLIP ViT-B/16) and a held-out annotator (C-AUROC$_L$, CLIP ViT-L/14); accuracy after 10 uncertainty-ordered reveals; accuracy after all reveals; and Int-AUC when interventions use ViT-L/14 labels (annotator shift).}
\label{tab:lf_fid_c10}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccc}
\toprule
Labels & Model & C-AUROC$_B$ & C-AUROC$_L$ & Acc@10$_{unc}$ & Acc@all & Int-AUC$_L$ \\
\midrule
\multirow{5}{*}{Complete} & LC-CBM (ours) & \textbf{0.885{\scriptsize$\pm$0.000}} & \textbf{0.644{\scriptsize$\pm$0.001}} & \textbf{0.894{\scriptsize$\pm$0.001}} & \textbf{0.894{\scriptsize$\pm$0.001}} & \textbf{0.719{\scriptsize$\pm$0.002}} \\
 & LF-SCBM (IS) & 0.861{\scriptsize$\pm$0.008} & 0.637{\scriptsize$\pm$0.004} & 0.873{\scriptsize$\pm$0.009} & 0.893{\scriptsize$\pm$0.004} & 0.686{\scriptsize$\pm$0.022} \\
 & LF-SCBM (CI) & 0.856{\scriptsize$\pm$0.008} & 0.635{\scriptsize$\pm$0.004} & 0.860{\scriptsize$\pm$0.013} & 0.893{\scriptsize$\pm$0.004} & 0.688{\scriptsize$\pm$0.019} \\
 & CBM & 0.883{\scriptsize$\pm$0.001} & \textbf{0.644{\scriptsize$\pm$0.001}} & 0.883{\scriptsize$\pm$0.002} & 0.893{\scriptsize$\pm$0.002} & 0.718{\scriptsize$\pm$0.000} \\
 & LF-CBM & 0.616{\scriptsize$\pm$0.001} & 0.608{\scriptsize$\pm$0.001} & 0.824{\scriptsize$\pm$0.003} & 0.247{\scriptsize$\pm$0.003} & 0.636{\scriptsize$\pm$0.003} \\
\midrule
\multirow{5}{*}{$\rho=0.3$} & LC-CBM (ours) & \textbf{0.874{\scriptsize$\pm$0.001}} & \textbf{0.642{\scriptsize$\pm$0.001}} & \textbf{0.888{\scriptsize$\pm$0.003}} & 0.870{\scriptsize$\pm$0.001} & 0.720{\scriptsize$\pm$0.012} \\
 & LF-SCBM (IS) & 0.855{\scriptsize$\pm$0.002} & 0.637{\scriptsize$\pm$0.001} & 0.874{\scriptsize$\pm$0.004} & \textbf{0.871{\scriptsize$\pm$0.007}} & 0.703{\scriptsize$\pm$0.015} \\
 & LF-SCBM (CI) & 0.845{\scriptsize$\pm$0.002} & 0.633{\scriptsize$\pm$0.001} & 0.861{\scriptsize$\pm$0.006} & \textbf{0.871{\scriptsize$\pm$0.007}} & 0.685{\scriptsize$\pm$0.019} \\
 & CBM & 0.871{\scriptsize$\pm$0.001} & 0.639{\scriptsize$\pm$0.003} & 0.880{\scriptsize$\pm$0.003} & 0.870{\scriptsize$\pm$0.004} & \textbf{0.732{\scriptsize$\pm$0.005}} \\
 & LF-CBM & 0.599{\scriptsize$\pm$0.002} & 0.595{\scriptsize$\pm$0.001} & 0.832{\scriptsize$\pm$0.006} & 0.262{\scriptsize$\pm$0.016} & 0.645{\scriptsize$\pm$0.008} \\
\midrule
\multirow{5}{*}{$\rho=0.1$} & LC-CBM (ours) & \textbf{0.857{\scriptsize$\pm$0.003}} & \textbf{0.634{\scriptsize$\pm$0.002}} & \textbf{0.891{\scriptsize$\pm$0.004}} & \textbf{0.853{\scriptsize$\pm$0.006}} & \textbf{0.739{\scriptsize$\pm$0.005}} \\
 & LF-SCBM (IS) & 0.835{\scriptsize$\pm$0.002} & 0.629{\scriptsize$\pm$0.003} & 0.873{\scriptsize$\pm$0.000} & 0.840{\scriptsize$\pm$0.006} & 0.700{\scriptsize$\pm$0.018} \\
 & LF-SCBM (CI) & 0.821{\scriptsize$\pm$0.003} & 0.623{\scriptsize$\pm$0.004} & 0.858{\scriptsize$\pm$0.005} & 0.840{\scriptsize$\pm$0.006} & 0.680{\scriptsize$\pm$0.010} \\
 & CBM & 0.852{\scriptsize$\pm$0.002} & 0.633{\scriptsize$\pm$0.001} & 0.879{\scriptsize$\pm$0.001} & 0.839{\scriptsize$\pm$0.005} & 0.733{\scriptsize$\pm$0.004} \\
 & LF-CBM & 0.581{\scriptsize$\pm$0.002} & 0.582{\scriptsize$\pm$0.004} & 0.821{\scriptsize$\pm$0.011} & 0.248{\scriptsize$\pm$0.022} & 0.621{\scriptsize$\pm$0.002} \\
\midrule
\multirow{5}{*}{$\rho=0.03$} & LC-CBM (ours) & \textbf{0.818{\scriptsize$\pm$0.004}} & \textbf{0.623{\scriptsize$\pm$0.001}} & \textbf{0.883{\scriptsize$\pm$0.001}} & \textbf{0.793{\scriptsize$\pm$0.005}} & 0.726{\scriptsize$\pm$0.019} \\
 & LF-SCBM (IS) & 0.778{\scriptsize$\pm$0.006} & 0.611{\scriptsize$\pm$0.002} & 0.879{\scriptsize$\pm$0.001} & 0.756{\scriptsize$\pm$0.018} & 0.680{\scriptsize$\pm$0.029} \\
 & LF-SCBM (CI) & 0.763{\scriptsize$\pm$0.004} & 0.606{\scriptsize$\pm$0.002} & 0.877{\scriptsize$\pm$0.002} & 0.756{\scriptsize$\pm$0.018} & 0.686{\scriptsize$\pm$0.020} \\
 & CBM & 0.815{\scriptsize$\pm$0.001} & 0.620{\scriptsize$\pm$0.002} & \textbf{0.883{\scriptsize$\pm$0.002}} & 0.789{\scriptsize$\pm$0.005} & \textbf{0.741{\scriptsize$\pm$0.009}} \\
 & LF-CBM & 0.558{\scriptsize$\pm$0.003} & 0.560{\scriptsize$\pm$0.002} & 0.832{\scriptsize$\pm$0.001} & 0.273{\scriptsize$\pm$0.016} & 0.615{\scriptsize$\pm$0.007} \\
\midrule
\multirow{5}{*}{10\% images} & LC-CBM (ours) & 0.836{\scriptsize$\pm$0.006} & \textbf{0.631{\scriptsize$\pm$0.003}} & \textbf{0.889{\scriptsize$\pm$0.004}} & 0.811{\scriptsize$\pm$0.011} & \textbf{0.733{\scriptsize$\pm$0.011}} \\
 & LF-SCBM (IS) & 0.791{\scriptsize$\pm$0.004} & 0.615{\scriptsize$\pm$0.002} & 0.868{\scriptsize$\pm$0.004} & \textbf{0.851{\scriptsize$\pm$0.003}} & 0.694{\scriptsize$\pm$0.033} \\
 & LF-SCBM (CI) & 0.783{\scriptsize$\pm$0.002} & 0.612{\scriptsize$\pm$0.001} & 0.857{\scriptsize$\pm$0.004} & \textbf{0.851{\scriptsize$\pm$0.003}} & 0.692{\scriptsize$\pm$0.031} \\
 & CBM & \textbf{0.844{\scriptsize$\pm$0.003}} & \textbf{0.631{\scriptsize$\pm$0.003}} & 0.866{\scriptsize$\pm$0.010} & 0.838{\scriptsize$\pm$0.018} & 0.721{\scriptsize$\pm$0.004} \\
 & LF-CBM & 0.581{\scriptsize$\pm$0.004} & 0.581{\scriptsize$\pm$0.002} & 0.813{\scriptsize$\pm$0.013} & 0.258{\scriptsize$\pm$0.032} & 0.631{\scriptsize$\pm$0.003} \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/lf/fidelity_c100.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{CIFAR-100: concept fidelity against the training annotator (C-AUROC$_B$, CLIP ViT-B/16) and a held-out annotator (C-AUROC$_L$, CLIP ViT-L/14); accuracy after 10 uncertainty-ordered reveals; accuracy after all reveals; and Int-AUC when interventions use ViT-L/14 labels (annotator shift). $\alpha=1$.}
\label{tab:lf_fid_c100}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccc}
\toprule
Labels & Model & C-AUROC$_B$ & C-AUROC$_L$ & Acc@10$_{unc}$ & Acc@all & Int-AUC$_L$ \\
\midrule
\multirow{5}{*}{Complete} & LC-CBM (ours) & \textbf{0.877{\scriptsize$\pm$0.000}} & \textbf{0.647{\scriptsize$\pm$0.000}} & \textbf{0.668{\scriptsize$\pm$0.000}} & 0.702{\scriptsize$\pm$0.003} & 0.592{\scriptsize$\pm$0.005} \\
 & LF-SCBM (IS) & 0.873{\scriptsize$\pm$0.000} & 0.645{\scriptsize$\pm$0.001} & 0.654{\scriptsize$\pm$0.004} & 0.701{\scriptsize$\pm$0.004} & 0.606{\scriptsize$\pm$0.009} \\
 & LF-SCBM (CI) & 0.872{\scriptsize$\pm$0.000} & 0.645{\scriptsize$\pm$0.001} & 0.645{\scriptsize$\pm$0.002} & \textbf{0.705{\scriptsize$\pm$0.004}} & \textbf{0.627{\scriptsize$\pm$0.003}} \\
 & CBM & 0.875{\scriptsize$\pm$0.001} & \textbf{0.647{\scriptsize$\pm$0.001}} & 0.632{\scriptsize$\pm$0.002} & 0.684{\scriptsize$\pm$0.002} & 0.606{\scriptsize$\pm$0.002} \\
 & LF-CBM & 0.629{\scriptsize$\pm$0.000} & 0.585{\scriptsize$\pm$0.000} & 0.645{\scriptsize$\pm$0.002} & 0.521{\scriptsize$\pm$0.002} & 0.578{\scriptsize$\pm$0.001} \\
\midrule
\multirow{5}{*}{$\rho=0.3$} & LC-CBM (ours) & \textbf{0.868{\scriptsize$\pm$0.001}} & \textbf{0.644{\scriptsize$\pm$0.000}} & \textbf{0.661{\scriptsize$\pm$0.001}} & \textbf{0.702{\scriptsize$\pm$0.002}} & 0.597{\scriptsize$\pm$0.007} \\
 & LF-SCBM (IS) & 0.865{\scriptsize$\pm$0.001} & 0.643{\scriptsize$\pm$0.000} & 0.630{\scriptsize$\pm$0.005} & 0.671{\scriptsize$\pm$0.005} & 0.593{\scriptsize$\pm$0.010} \\
 & LF-SCBM (CI) & 0.865{\scriptsize$\pm$0.001} & 0.642{\scriptsize$\pm$0.000} & 0.624{\scriptsize$\pm$0.002} & 0.673{\scriptsize$\pm$0.006} & 0.606{\scriptsize$\pm$0.004} \\
 & CBM & 0.866{\scriptsize$\pm$0.000} & 0.643{\scriptsize$\pm$0.000} & 0.636{\scriptsize$\pm$0.004} & 0.684{\scriptsize$\pm$0.004} & \textbf{0.617{\scriptsize$\pm$0.004}} \\
 & LF-CBM & 0.607{\scriptsize$\pm$0.000} & 0.572{\scriptsize$\pm$0.001} & 0.636{\scriptsize$\pm$0.003} & 0.520{\scriptsize$\pm$0.003} & 0.575{\scriptsize$\pm$0.002} \\
\midrule
\multirow{5}{*}{$\rho=0.1$} & LC-CBM (ours) & \textbf{0.856{\scriptsize$\pm$0.000}} & \textbf{0.640{\scriptsize$\pm$0.001}} & 0.620{\scriptsize$\pm$0.006} & \textbf{0.649{\scriptsize$\pm$0.010}} & 0.579{\scriptsize$\pm$0.017} \\
 & LF-SCBM (IS) & 0.851{\scriptsize$\pm$0.001} & 0.639{\scriptsize$\pm$0.001} & 0.598{\scriptsize$\pm$0.003} & 0.630{\scriptsize$\pm$0.002} & 0.569{\scriptsize$\pm$0.011} \\
 & LF-SCBM (CI) & 0.851{\scriptsize$\pm$0.001} & 0.638{\scriptsize$\pm$0.001} & 0.594{\scriptsize$\pm$0.005} & 0.631{\scriptsize$\pm$0.004} & 0.576{\scriptsize$\pm$0.005} \\
 & CBM & 0.850{\scriptsize$\pm$0.000} & 0.638{\scriptsize$\pm$0.001} & 0.609{\scriptsize$\pm$0.003} & 0.647{\scriptsize$\pm$0.007} & \textbf{0.596{\scriptsize$\pm$0.004}} \\
 & LF-CBM & 0.581{\scriptsize$\pm$0.001} & 0.557{\scriptsize$\pm$0.001} & \textbf{0.632{\scriptsize$\pm$0.001}} & 0.527{\scriptsize$\pm$0.006} & 0.577{\scriptsize$\pm$0.003} \\
\midrule
\multirow{5}{*}{$\rho=0.03$} & LC-CBM (ours) & \textbf{0.827{\scriptsize$\pm$0.001}} & \textbf{0.630{\scriptsize$\pm$0.000}} & 0.600{\scriptsize$\pm$0.004} & \textbf{0.611{\scriptsize$\pm$0.004}} & 0.566{\scriptsize$\pm$0.008} \\
 & LF-SCBM (IS) & 0.821{\scriptsize$\pm$0.001} & 0.629{\scriptsize$\pm$0.001} & 0.585{\scriptsize$\pm$0.008} & 0.594{\scriptsize$\pm$0.003} & 0.563{\scriptsize$\pm$0.003} \\
 & LF-SCBM (CI) & 0.821{\scriptsize$\pm$0.001} & 0.629{\scriptsize$\pm$0.001} & 0.574{\scriptsize$\pm$0.006} & 0.590{\scriptsize$\pm$0.007} & 0.560{\scriptsize$\pm$0.007} \\
 & CBM & 0.820{\scriptsize$\pm$0.000} & 0.628{\scriptsize$\pm$0.001} & 0.578{\scriptsize$\pm$0.011} & 0.599{\scriptsize$\pm$0.009} & \textbf{0.568{\scriptsize$\pm$0.011}} \\
 & LF-CBM & 0.552{\scriptsize$\pm$0.001} & 0.539{\scriptsize$\pm$0.001} & \textbf{0.619{\scriptsize$\pm$0.001}} & 0.515{\scriptsize$\pm$0.003} & 0.565{\scriptsize$\pm$0.003} \\
\midrule
\multirow{5}{*}{10\% images} & LC-CBM (ours) & 0.830{\scriptsize$\pm$0.004} & 0.632{\scriptsize$\pm$0.003} & 0.618{\scriptsize$\pm$0.013} & \textbf{0.629{\scriptsize$\pm$0.018}} & \textbf{0.597{\scriptsize$\pm$0.018}} \\
 & LF-SCBM (IS) & \textbf{0.840{\scriptsize$\pm$0.000}} & \textbf{0.636{\scriptsize$\pm$0.001}} & 0.575{\scriptsize$\pm$0.011} & 0.601{\scriptsize$\pm$0.011} & 0.540{\scriptsize$\pm$0.006} \\
 & LF-SCBM (CI) & 0.839{\scriptsize$\pm$0.000} & \textbf{0.636{\scriptsize$\pm$0.001}} & 0.566{\scriptsize$\pm$0.014} & 0.601{\scriptsize$\pm$0.012} & 0.549{\scriptsize$\pm$0.014} \\
 & CBM & 0.837{\scriptsize$\pm$0.001} & 0.633{\scriptsize$\pm$0.001} & 0.544{\scriptsize$\pm$0.012} & 0.586{\scriptsize$\pm$0.011} & 0.532{\scriptsize$\pm$0.011} \\
 & LF-CBM & 0.585{\scriptsize$\pm$0.002} & 0.558{\scriptsize$\pm$0.001} & \textbf{0.623{\scriptsize$\pm$0.003}} & 0.521{\scriptsize$\pm$0.002} & 0.569{\scriptsize$\pm$0.003} \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/lf/main_c10.tex <==
\begin{table*}[h]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{CIFAR-10 with incomplete concept labels (mean$\pm$sd over 3 seeds). Bold: best per column within each label setting.}
\label{tab:lf_main_c10}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccccc}
\toprule
Labels & Model & Acc@0 & Acc@10 & Acc@50 & Int-AUC & Imp-AUROC & Joint NLL$\downarrow$ \\
\midrule
\multirow{3}{*}{Complete} & LC-CBM (ours) & \textbf{0.877{\scriptsize$\pm$0.002}} & \textbf{0.885{\scriptsize$\pm$0.001}} & \textbf{0.899{\scriptsize$\pm$0.001}} & \textbf{0.896{\scriptsize$\pm$0.001}} & \textbf{0.961{\scriptsize$\pm$0.000}} & \textbf{30.2{\scriptsize$\pm$0.0}} \\
 & CBM & 0.868{\scriptsize$\pm$0.003} & 0.874{\scriptsize$\pm$0.002} & 0.893{\scriptsize$\pm$0.001} & 0.892{\scriptsize$\pm$0.002} & 0.945{\scriptsize$\pm$0.000} & 40.8{\scriptsize$\pm$0.0} \\
 & LF-CBM & 0.867{\scriptsize$\pm$0.000} & 0.851{\scriptsize$\pm$0.001} & 0.778{\scriptsize$\pm$0.001} & 0.665{\scriptsize$\pm$0.003} & 0.884{\scriptsize$\pm$0.000} & -- \\
\midrule
\multirow{3}{*}{$\rho=0.3$} & LC-CBM (ours) & \textbf{0.875{\scriptsize$\pm$0.001}} & \textbf{0.882{\scriptsize$\pm$0.002}} & \textbf{0.890{\scriptsize$\pm$0.002}} & \textbf{0.884{\scriptsize$\pm$0.001}} & \textbf{0.956{\scriptsize$\pm$0.002}} & \textbf{32.6{\scriptsize$\pm$0.0}} \\
 & CBM & 0.866{\scriptsize$\pm$0.004} & 0.873{\scriptsize$\pm$0.003} & \textbf{0.890{\scriptsize$\pm$0.003}} & \textbf{0.884{\scriptsize$\pm$0.004}} & 0.941{\scriptsize$\pm$0.000} & 42.1{\scriptsize$\pm$0.0} \\
 & LF-CBM & 0.861{\scriptsize$\pm$0.003} & 0.848{\scriptsize$\pm$0.002} & 0.783{\scriptsize$\pm$0.002} & 0.677{\scriptsize$\pm$0.004} & 0.881{\scriptsize$\pm$0.000} & -- \\
\midrule
\multirow{3}{*}{$\rho=0.1$} & LC-CBM (ours) & \textbf{0.878{\scriptsize$\pm$0.003}} & \textbf{0.884{\scriptsize$\pm$0.002}} & \textbf{0.894{\scriptsize$\pm$0.003}} & \textbf{0.883{\scriptsize$\pm$0.004}} & \textbf{0.944{\scriptsize$\pm$0.002}} & \textbf{37.1{\scriptsize$\pm$0.0}} \\
 & CBM & 0.865{\scriptsize$\pm$0.001} & 0.871{\scriptsize$\pm$0.001} & 0.885{\scriptsize$\pm$0.002} & 0.873{\scriptsize$\pm$0.002} & 0.935{\scriptsize$\pm$0.000} & 44.9{\scriptsize$\pm$0.2} \\
 & LF-CBM & 0.855{\scriptsize$\pm$0.000} & 0.840{\scriptsize$\pm$0.001} & 0.765{\scriptsize$\pm$0.004} & 0.655{\scriptsize$\pm$0.000} & 0.878{\scriptsize$\pm$0.000} & -- \\
\midrule
\multirow{3}{*}{$\rho=0.03$} & LC-CBM (ours) & \textbf{0.879{\scriptsize$\pm$0.002}} & \textbf{0.883{\scriptsize$\pm$0.001}} & 0.875{\scriptsize$\pm$0.005} & 0.856{\scriptsize$\pm$0.004} & \textbf{0.933{\scriptsize$\pm$0.002}} & \textbf{45.5{\scriptsize$\pm$0.3}} \\
 & CBM & 0.874{\scriptsize$\pm$0.002} & 0.877{\scriptsize$\pm$0.002} & \textbf{0.885{\scriptsize$\pm$0.002}} & \textbf{0.862{\scriptsize$\pm$0.002}} & 0.920{\scriptsize$\pm$0.000} & 51.9{\scriptsize$\pm$0.2} \\
 & LF-CBM & 0.848{\scriptsize$\pm$0.001} & 0.831{\scriptsize$\pm$0.003} & 0.754{\scriptsize$\pm$0.006} & 0.650{\scriptsize$\pm$0.003} & 0.876{\scriptsize$\pm$0.001} & -- \\
\midrule
\multirow{3}{*}{10\% images} & LC-CBM (ours) & \textbf{0.882{\scriptsize$\pm$0.001}} & \textbf{0.884{\scriptsize$\pm$0.001}} & \textbf{0.884{\scriptsize$\pm$0.008}} & 0.864{\scriptsize$\pm$0.003} & \textbf{0.939{\scriptsize$\pm$0.007}} & \textbf{36.2{\scriptsize$\pm$0.3}} \\
 & CBM & 0.853{\scriptsize$\pm$0.009} & 0.859{\scriptsize$\pm$0.009} & 0.876{\scriptsize$\pm$0.009} & \textbf{0.866{\scriptsize$\pm$0.012}} & 0.932{\scriptsize$\pm$0.000} & 45.9{\scriptsize$\pm$0.4} \\
 & LF-CBM & 0.850{\scriptsize$\pm$0.001} & 0.837{\scriptsize$\pm$0.001} & 0.767{\scriptsize$\pm$0.006} & 0.662{\scriptsize$\pm$0.009} & 0.879{\scriptsize$\pm$0.000} & -- \\
\bottomrule
\end{tabular}}
\end{table*}

==> tables/lf/main_c100.tex <==
\begin{table*}[h]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{CIFAR-100 with incomplete concept labels (mean$\pm$sd over 3 seeds, $\alpha=1$). Bold: best per column within each label setting.}
\label{tab:lf_main_c100}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccccc}
\toprule
Labels & Model & Acc@0 & Acc@10 & Acc@50 & Int-AUC & Imp-AUROC & Joint NLL$\downarrow$ \\
\midrule
\multirow{3}{*}{Complete} & LC-CBM (ours) & \textbf{0.655{\scriptsize$\pm$0.001}} & \textbf{0.659{\scriptsize$\pm$0.002}} & \textbf{0.675{\scriptsize$\pm$0.002}} & \textbf{0.683{\scriptsize$\pm$0.002}} & \textbf{0.960{\scriptsize$\pm$0.002}} & \textbf{194.8{\scriptsize$\pm$0.1}} \\
 & CBM & 0.620{\scriptsize$\pm$0.002} & 0.626{\scriptsize$\pm$0.002} & 0.640{\scriptsize$\pm$0.001} & 0.655{\scriptsize$\pm$0.001} & 0.944{\scriptsize$\pm$0.000} & 260.2{\scriptsize$\pm$0.5} \\
 & LF-CBM & 0.648{\scriptsize$\pm$0.001} & 0.640{\scriptsize$\pm$0.001} & 0.612{\scriptsize$\pm$0.002} & 0.581{\scriptsize$\pm$0.000} & 0.891{\scriptsize$\pm$0.000} & -- \\
\midrule
\multirow{3}{*}{$\rho=0.3$} & LC-CBM (ours) & \textbf{0.642{\scriptsize$\pm$0.000}} & \textbf{0.649{\scriptsize$\pm$0.001}} & \textbf{0.666{\scriptsize$\pm$0.002}} & \textbf{0.678{\scriptsize$\pm$0.001}} & \textbf{0.956{\scriptsize$\pm$0.001}} & \textbf{209.9{\scriptsize$\pm$0.1}} \\
 & CBM & 0.626{\scriptsize$\pm$0.004} & 0.632{\scriptsize$\pm$0.003} & 0.644{\scriptsize$\pm$0.003} & 0.657{\scriptsize$\pm$0.004} & 0.941{\scriptsize$\pm$0.000} & 266.1{\scriptsize$\pm$0.2} \\
 & LF-CBM & 0.639{\scriptsize$\pm$0.003} & 0.632{\scriptsize$\pm$0.002} & 0.606{\scriptsize$\pm$0.002} & 0.579{\scriptsize$\pm$0.002} & 0.888{\scriptsize$\pm$0.000} & -- \\
\midrule
\multirow{3}{*}{$\rho=0.1$} & LC-CBM (ours) & 0.609{\scriptsize$\pm$0.007} & 0.614{\scriptsize$\pm$0.007} & \textbf{0.626{\scriptsize$\pm$0.009}} & \textbf{0.634{\scriptsize$\pm$0.009}} & \textbf{0.947{\scriptsize$\pm$0.003}} & \textbf{230.0{\scriptsize$\pm$0.1}} \\
 & CBM & 0.603{\scriptsize$\pm$0.004} & 0.606{\scriptsize$\pm$0.005} & 0.616{\scriptsize$\pm$0.005} & 0.625{\scriptsize$\pm$0.005} & 0.937{\scriptsize$\pm$0.000} & 277.7{\scriptsize$\pm$0.3} \\
 & LF-CBM & \textbf{0.634{\scriptsize$\pm$0.002}} & \textbf{0.630{\scriptsize$\pm$0.001}} & 0.608{\scriptsize$\pm$0.000} & 0.582{\scriptsize$\pm$0.003} & 0.885{\scriptsize$\pm$0.000} & -- \\
\midrule
\multirow{3}{*}{$\rho=0.03$} & LC-CBM (ours) & 0.592{\scriptsize$\pm$0.004} & 0.593{\scriptsize$\pm$0.005} & \textbf{0.601{\scriptsize$\pm$0.005}} & \textbf{0.603{\scriptsize$\pm$0.005}} & \textbf{0.938{\scriptsize$\pm$0.002}} & \textbf{264.2{\scriptsize$\pm$0.2}} \\
 & CBM & 0.576{\scriptsize$\pm$0.011} & 0.577{\scriptsize$\pm$0.011} & 0.581{\scriptsize$\pm$0.011} & 0.588{\scriptsize$\pm$0.010} & 0.927{\scriptsize$\pm$0.000} & 301.6{\scriptsize$\pm$1.2} \\
 & LF-CBM & \textbf{0.623{\scriptsize$\pm$0.002}} & \textbf{0.617{\scriptsize$\pm$0.002}} & 0.595{\scriptsize$\pm$0.002} & 0.569{\scriptsize$\pm$0.002} & 0.882{\scriptsize$\pm$0.000} & -- \\
\midrule
\multirow{3}{*}{10\% images} & LC-CBM (ours) & 0.612{\scriptsize$\pm$0.012} & 0.613{\scriptsize$\pm$0.012} & \textbf{0.619{\scriptsize$\pm$0.017}} & \textbf{0.622{\scriptsize$\pm$0.017}} & \textbf{0.933{\scriptsize$\pm$0.001}} & \textbf{236.3{\scriptsize$\pm$2.9}} \\
 & CBM & 0.537{\scriptsize$\pm$0.012} & 0.541{\scriptsize$\pm$0.014} & 0.549{\scriptsize$\pm$0.013} & 0.562{\scriptsize$\pm$0.012} & 0.932{\scriptsize$\pm$0.000} & 288.4{\scriptsize$\pm$0.3} \\
 & LF-CBM & \textbf{0.627{\scriptsize$\pm$0.002}} & \textbf{0.622{\scriptsize$\pm$0.002}} & 0.598{\scriptsize$\pm$0.004} & 0.573{\scriptsize$\pm$0.003} & 0.885{\scriptsize$\pm$0.000} & -- \\
\bottomrule
\end{tabular}}
\end{table*}

==> tables/lf/soft_c10.tex <==
\begin{table*}[t]
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{CIFAR-10: soft concept targets $t=\sigma(100\,(s_c-s_{\neg c}))$ (CLIP two-prompt probability) versus binary targets $\mathbb{1}[t>0.5]$. Acc@all: accuracy after revealing all 143 concepts.}
\label{tab:lf_soft}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccc}
\toprule
Labels & Model & Acc@0 & Acc@10 & Acc@50 & Acc@all & Int-AUC \\
\midrule
\multirow{5}{*}{Complete} & LC-CBM-soft (ours) & 0.875{\scriptsize$\pm$0.001} & 0.877{\scriptsize$\pm$0.002} & 0.866{\scriptsize$\pm$0.003} & 0.839{\scriptsize$\pm$0.001} & 0.858{\scriptsize$\pm$0.002} \\
 & CBM-soft & 0.860{\scriptsize$\pm$0.002} & 0.859{\scriptsize$\pm$0.002} & 0.852{\scriptsize$\pm$0.001} & 0.842{\scriptsize$\pm$0.001} & 0.850{\scriptsize$\pm$0.001} \\
 & LC-CBM (ours) & \textbf{0.877{\scriptsize$\pm$0.002}} & \textbf{0.885{\scriptsize$\pm$0.001}} & \textbf{0.899{\scriptsize$\pm$0.001}} & \textbf{0.894{\scriptsize$\pm$0.001}} & \textbf{0.896{\scriptsize$\pm$0.001}} \\
 & CBM & 0.868{\scriptsize$\pm$0.003} & 0.874{\scriptsize$\pm$0.002} & 0.893{\scriptsize$\pm$0.001} & 0.893{\scriptsize$\pm$0.002} & 0.892{\scriptsize$\pm$0.002} \\
 & LF-CBM & 0.867{\scriptsize$\pm$0.000} & 0.851{\scriptsize$\pm$0.001} & 0.778{\scriptsize$\pm$0.001} & 0.247{\scriptsize$\pm$0.003} & 0.665{\scriptsize$\pm$0.003} \\
\midrule
\multirow{5}{*}{$\rho=0.3$} & LC-CBM-soft (ours) & \textbf{0.892{\scriptsize$\pm$0.003}} & \textbf{0.898{\scriptsize$\pm$0.002}} & \textbf{0.902{\scriptsize$\pm$0.002}} & 0.823{\scriptsize$\pm$0.001} & 0.879{\scriptsize$\pm$0.002} \\
 & CBM-soft & 0.890{\scriptsize$\pm$0.001} & 0.893{\scriptsize$\pm$0.000} & 0.884{\scriptsize$\pm$0.001} & 0.825{\scriptsize$\pm$0.000} & 0.869{\scriptsize$\pm$0.000} \\
 & LC-CBM (ours) & 0.875{\scriptsize$\pm$0.001} & 0.882{\scriptsize$\pm$0.002} & 0.890{\scriptsize$\pm$0.002} & \textbf{0.870{\scriptsize$\pm$0.001}} & \textbf{0.884{\scriptsize$\pm$0.001}} \\
 & CBM & 0.866{\scriptsize$\pm$0.004} & 0.873{\scriptsize$\pm$0.003} & 0.890{\scriptsize$\pm$0.003} & \textbf{0.870{\scriptsize$\pm$0.004}} & \textbf{0.884{\scriptsize$\pm$0.004}} \\
 & LF-CBM & 0.861{\scriptsize$\pm$0.003} & 0.848{\scriptsize$\pm$0.002} & 0.783{\scriptsize$\pm$0.002} & 0.262{\scriptsize$\pm$0.016} & 0.677{\scriptsize$\pm$0.004} \\
\midrule
\multirow{5}{*}{$\rho=0.1$} & LC-CBM-soft (ours) & \textbf{0.895{\scriptsize$\pm$0.001}} & \textbf{0.901{\scriptsize$\pm$0.000}} & \textbf{0.909{\scriptsize$\pm$0.001}} & 0.791{\scriptsize$\pm$0.003} & 0.877{\scriptsize$\pm$0.001} \\
 & CBM-soft & 0.894{\scriptsize$\pm$0.002} & 0.899{\scriptsize$\pm$0.002} & 0.897{\scriptsize$\pm$0.001} & 0.800{\scriptsize$\pm$0.005} & 0.871{\scriptsize$\pm$0.002} \\
 & LC-CBM (ours) & 0.878{\scriptsize$\pm$0.003} & 0.884{\scriptsize$\pm$0.002} & 0.894{\scriptsize$\pm$0.003} & \textbf{0.853{\scriptsize$\pm$0.006}} & \textbf{0.883{\scriptsize$\pm$0.004}} \\
 & CBM & 0.865{\scriptsize$\pm$0.001} & 0.871{\scriptsize$\pm$0.001} & 0.885{\scriptsize$\pm$0.002} & 0.839{\scriptsize$\pm$0.005} & 0.873{\scriptsize$\pm$0.002} \\
 & LF-CBM & 0.855{\scriptsize$\pm$0.000} & 0.840{\scriptsize$\pm$0.001} & 0.765{\scriptsize$\pm$0.004} & 0.248{\scriptsize$\pm$0.022} & 0.655{\scriptsize$\pm$0.000} \\
\midrule
\multirow{5}{*}{$\rho=0.03$} & LC-CBM-soft (ours) & 0.892{\scriptsize$\pm$0.001} & 0.897{\scriptsize$\pm$0.000} & \textbf{0.907{\scriptsize$\pm$0.001}} & 0.736{\scriptsize$\pm$0.011} & \textbf{0.866{\scriptsize$\pm$0.002}} \\
 & CBM-soft & \textbf{0.898{\scriptsize$\pm$0.001}} & \textbf{0.899{\scriptsize$\pm$0.001}} & 0.899{\scriptsize$\pm$0.002} & 0.735{\scriptsize$\pm$0.020} & 0.860{\scriptsize$\pm$0.006} \\
 & LC-CBM (ours) & 0.879{\scriptsize$\pm$0.002} & 0.883{\scriptsize$\pm$0.001} & 0.875{\scriptsize$\pm$0.005} & \textbf{0.793{\scriptsize$\pm$0.005}} & 0.856{\scriptsize$\pm$0.004} \\
 & CBM & 0.874{\scriptsize$\pm$0.002} & 0.877{\scriptsize$\pm$0.002} & 0.885{\scriptsize$\pm$0.002} & 0.789{\scriptsize$\pm$0.005} & 0.862{\scriptsize$\pm$0.002} \\
 & LF-CBM & 0.848{\scriptsize$\pm$0.001} & 0.831{\scriptsize$\pm$0.003} & 0.754{\scriptsize$\pm$0.006} & 0.273{\scriptsize$\pm$0.016} & 0.650{\scriptsize$\pm$0.003} \\
\midrule
\multirow{5}{*}{10\% images} & LC-CBM-soft (ours) & \textbf{0.890{\scriptsize$\pm$0.002}} & \textbf{0.895{\scriptsize$\pm$0.002}} & 0.895{\scriptsize$\pm$0.005} & 0.786{\scriptsize$\pm$0.011} & 0.865{\scriptsize$\pm$0.006} \\
 & CBM-soft & 0.887{\scriptsize$\pm$0.002} & 0.892{\scriptsize$\pm$0.002} & \textbf{0.897{\scriptsize$\pm$0.002}} & 0.812{\scriptsize$\pm$0.001} & \textbf{0.874{\scriptsize$\pm$0.001}} \\
 & LC-CBM (ours) & 0.882{\scriptsize$\pm$0.001} & 0.884{\scriptsize$\pm$0.001} & 0.884{\scriptsize$\pm$0.008} & 0.811{\scriptsize$\pm$0.011} & 0.864{\scriptsize$\pm$0.003} \\
 & CBM & 0.853{\scriptsize$\pm$0.009} & 0.859{\scriptsize$\pm$0.009} & 0.876{\scriptsize$\pm$0.009} & \textbf{0.838{\scriptsize$\pm$0.018}} & 0.866{\scriptsize$\pm$0.012} \\
 & LF-CBM & 0.850{\scriptsize$\pm$0.001} & 0.837{\scriptsize$\pm$0.001} & 0.767{\scriptsize$\pm$0.006} & 0.258{\scriptsize$\pm$0.032} & 0.662{\scriptsize$\pm$0.009} \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/paired.tex <==
\begin{tabular}{lcccc}
\toprule
Dataset & Pairs & $\Delta$ Concept acc. & $\Delta$ Target acc. & $\Delta$ AUC (unc.) \\
\midrule
Synthetic & 10 & +0.26{\scriptsize$\pm$0.23} ($p{=}0.007$, 9/10) & +0.11{\scriptsize$\pm$0.62} ($p{=}0.590$, 5/10) & +2.08{\scriptsize$\pm$0.49} ($p{<}10^{-3}$, 10/10) \\
CUB & 10 & +0.63{\scriptsize$\pm$0.09} ($p{<}10^{-3}$, 10/10) & +2.51{\scriptsize$\pm$0.65} ($p{<}10^{-3}$, 10/10) & +1.35{\scriptsize$\pm$0.15} ($p{<}10^{-3}$, 10/10) \\
CIFAR-10 & 10 & +0.55{\scriptsize$\pm$0.05} ($p{<}10^{-3}$, 10/10) & +0.58{\scriptsize$\pm$0.30} ($p{<}10^{-3}$, 10/10) & +1.48{\scriptsize$\pm$0.14} ($p{<}10^{-3}$, 10/10) \\
CIFAR-100 & 3 & -0.26{\scriptsize$\pm$0.09} ($p{=}0.038$, 0/3) & +1.71{\scriptsize$\pm$1.32} ($p{=}0.155$, 3/3) & +2.58{\scriptsize$\pm$0.87} ($p{=}0.036$, 3/3) \\
\bottomrule
\end{tabular}

